An Unsupervised Cross-Modal Hashing Method Robust to Noisy Training Image-Text Correspondences in Remote Sensing

The development of accurate and scalable cross-modal image-text retrieval methods, where queries from one modality (e.g., text) can be matched to archive entries from another (e.g., remote sensing image) has attracted great attention in remote sensing (RS). Most of the existing methods assume that a reliable multi-modal training set with accurately matched text-image pairs is existing. However, this assumption may not always hold since the multi-modal training sets may include noisy pairs (i.e., textual descriptions/captions associated to training images can be noisy), distorting the learning process of the retrieval methods. To address this problem, we propose a novel unsupervised cross-modal hashing method robust to the noisy image-text correspondences (CHNR). CHNR consists of three modules: 1) feature extraction module, which extracts feature representations of image-text pairs; 2) noise detection module, which detects potential noisy correspondences; and 3) hashing module that generates cross-modal binary hash codes. The proposed CHNR includes two training phases: i) meta-learning phase that uses a small portion of clean (i.e., reliable) data to train the noise detection module in an adversarial fashion; and ii) the main training phase for which the trained noise detection module is used to identify noisy correspondences while the hashing module is trained on the noisy multi-modal training set. Experimental results show that the proposed CHNR outperforms state-of-the-art methods. Our code is publicly available at https://git.tu-berlin.de/rsim/chnr

==> sections/4_results.tex <==


\noindent\textbf{Comparison of the proposed method with different cross-
modal retrieval methods}. We evaluated the effectiveness of the proposed CHNR method compared to different supervised and unsupervised cross-modal retrieval methods, which are: DJSRH \cite{su2019deep} and JDSH \cite{liu2020joint} (see Section \ref{sec:intro} for the details about each method). We trained all models under the same experimental setup for a fair comparison. Results of each method are provided in terms of mean average precision assessed on top-20 retrieved images (mAP@20). The experiments are conducted over different injected noise rates (5\%, 10\%, 20\%, 30\%, 40\%, and 50\%) when $B=64$. Table \ref{tab:retrieval-results} shows the retrieval performance for RSICD and UCM datasets. From the table, one can observe that the proposed CHNR method sharply outperformed all the unsupervised baselines in $I \to T$  and $T \to I$ tasks for all injected noise rates on both datasets. As an example, for $I \to T$ retrieval task from UCM dataset, when the injected noise rate in 20\% the proposed CHNR obtained about 13\% and 21\% higher scores than JDSH and DJSRH, respectively. Similarly, for the RSICD dataset in $T \to I$ retrieval task when the injected noise rate is 20\%, the proposed CHNR outperformed JDSH and DJSRH with 5\% and 15\% higher mAP@20 scores, respectively. From the table, one can observe that all the compared methods are robust to small amounts of noise (i.e., $5\%$ and $10\%$), while the mAP@20 drops significantly for all methods by increasing the injected noise rate ( more than 20\% ) for  $I \to T$  and $T \to I$ tasks. However, the performance drop is considerably smaller for the proposed CHNR than the other methods. As an example, when the noise injection rate is $5\%$ for $I \to T$ task in RSICD dataset, the performance of CHNR is $2\%$ and $9\%$ higher than JDSH and DJSRH, respectively. However, when the injected noise rate increases to 50\% for the same task in the same dataset the performance of CHNR is $32\%$ and $31\%$ higher than JDSH and DJSRH, respectively.


%We evaluate the effectiveness of the proposed CHNR method compared to different supervised and unsupervised cross-modal retrieval methods, which are: DJSRH \cite{su2019deep} and JDSH \cite{liu2020joint} (see Section \ref{sec:intro} for the details about each method). For a fair comparison, we trained all models under the same experimental setup. Results of each method are provided in terms of mean average precision assessed on top-20 retrieved images (mAP@20). The experiments are conducted over different injected noise rates (5\%, 10\%, 20\%, 30\%, 40\%, and 50\%) when $B=64$. Table \ref{tab:retrieval-results} shows the retrieval performance for RSICD and UCM datasets. From the table one can observe that all the compared methods are robust to small amounts of noise ($5\%$ - $10\%$). The mAP@20 is decreasing for all methods with the injection of more noise, but the final performance drop is considerably smaller for methods with noise reduction (CHNR). For instance, when the noise injection rate is $20\%$ for RSICD dataset, the performance of CHNR-EW is $1,7\%$ higher than DUCH and $5,8\%$ higher than JDSH, when the noise injection rate is $40\%$, CHNR-EW performs $10.9\%$ and $22,6\%$ better respectively. The DUCH-family of methods also outperforms JDSH and DJSRH baselines. The CHNR-PTC model without the noise reduction but with initial-pretraining on clean data ($\textbf{O}_C$) outperforms the baseline DUCH model, trained on the complete dataset ($\textbf{O}$) from the first epoch. DUCH with noise reduction with exponential weights (CHNR-EW) and with discrete weights (CHNR-DW) are the most efficient models in the case of both datasets. In Fig. \ref{fig:retrieval-results} the visual representations of retrieval rates for RSICD and UCM are demonstrated.










%In the figure \ref{fig:weights} the distributions of clean and noisy image-text joint-feature pairs weights assigned by the noise discriminator are shown. The diagram is made for the noise injection rate of 50\%. Modes of clean and noisy weight data distributions are around $0.8$ and $0.1$ respectively. The distribution shape shows, that the noise discriminator is able to distinguish noisy and clean data effectively with minor mistakes.


%To analyze the influence of noise reduction methods, we tested different models from DUCH-family. Table \ref{tab:retrieval-results} and Fig. \ref{fig:retrieval-results} show the results of ablation study. In detail, we compared the default model (DUCH) and the model with pretraining on clean data only (CHNR-PTC) with noise reduction models (CHNR-NW, CHNR-EW, CHNR-DW). Default DUCH model is only robust to small amounts of noise in the data (up to 10\%). The CHNR-PTC is trained only on clean data for the first 75 epochs and the rest data (with noise) is added for the next 75 training epochs. The CHNR-PTC is slightly more robust to the noise (4\% - 7\% better in different tasks with 50\% of noisy data) than DUCH, but still outperformed by any of the methods with noise reduction. Models with noise reduction show the best performance, for 30\% noise case up to 5\% better for RSICD and up to 9\% better for UCM. For 50\% of noise case this performance difference is increased up to 18\% for RSICD and up to 21\% for UCM. CHNR-EW and CHNR-DW showed the best performance for both datasets, where CHNR-DW was more efficient in case of RSICD and CHNR-EW - in case of UCM. CHNR-NW was marginally worse than the other two noise reduction models in both experiments.

% CHNR-NW - noise detection + normal/natural weights (discriminator weights), nw = w
% CHNR-EW - noise detection + exponential weights (discriminator weights), ew = abs(w^3)
% CHNR-DW - noise detection + discrete weights (discriminator weights), w <= 0.5 --> dw = 0, w > 0.5 --> dw = 1
% CHNR-PTC - pre-train on clean data, 1. meta-learning on clean data, 2. all data, w = 1
% DUCH - default DUCH
% JDSH - default JDSH
% DJSRH - default DJSRH

==> sections/visuals_old.tex <==
\begin{table}[]
% see /data/plots_table_rsicd.csv
\setlength{\tabcolsep}{3pt}
\centering

\caption{The mAP@20 results for image-to-text ($I \to T$) and text-to-image ($T \to I$) retrieval for the RSICD dataset when $B=64$.}
\small
\label{tab:retrieval-rsicd}
\def\arraystretch{1.0}
\begin{tabular}{c|l|cccccc}
\hline
\multirow{2}{*}{Task} & \multirow{2}{*}{Metod} & \multicolumn{6}{c}{Amount of the caption noise} \\
 & & 5\% & 10\% & 20\% & 30\% & 40\% & 50\% \\
\hline\hline
\multirow{7}{*}{$I \to T$}
 & DUCH-NR-NW & 0.778 & 0.752 & 0.730 & 0.720 & 0.668 & 0.617 \\
 & DUCH-NR-EW & 0.742 & 0.723 & \textbf{0.741} & \underline{0.728} & \underline{0.713} & \underline{0.687} \\
 & DUCH-NR-DW & \textbf{0.786} & \textbf{0.770} & \underline{0.739} & \textbf{0.732} & \textbf{0.717} & \textbf{0.708} \\
\cline{2-8}
 & DUCH-PTC & 0.772 & 0.749 & 0.698 & 0.660 & 0.582 & 0.525 \\
 & DUCH & \underline{0.785} & \underline{0.767} & 0.724 & 0.677 & 0.604 & 0.475 \\
 & JDSH\cite{liu2020joint}& 0.768 & 0.737 & 0.683 & 0.609 & 0.487 & 0.381 \\
 & DJSRH\cite{su2019deep} & 0.669 & 0.661 & 0.602 & 0.559 & 0.491 & 0.397 \\
\hline\hline
\multirow{7}{*}{$T \to I$}
 & DUCH-NR-NW & 0.778 & 0.767 & 0.745 & 0.737 & 0.704 & 0.664 \\
 & DUCH-NR-EW & 0.747 & 0.752 & 0.746 & \underline{0.739} & \underline{0.718} & \underline{0.688} \\
 & DUCH-NR-DW & \underline{0.783} & \underline{0.782} & \textbf{0.754} & \textbf{0.746} & \textbf{0.720} & \textbf{0.718} \\
\cline{2-8}
 & DUCH-PTC & 0.776 & 0.766 & 0.727 & 0.709 & 0.648 & 0.614 \\
 & DUCH & \textbf{0.784} & \textbf{0.783} & \underline{0.751} & 0.706 & 0.647 & 0.540 \\
 & JDSH\cite{liu2020joint}& 0.769 & 0.754 & 0.699 & 0.639 & 0.540 & 0.415 \\
 & DJSRH\cite{su2019deep} & 0.666 & 0.647 & 0.600 & 0.547 & 0.472 & 0.373 \\
\hline
\end{tabular}
\end{table}


\begin{table}[]
% see /data/plots_table_ucm.csv
\setlength{\tabcolsep}{3pt}
\centering


\caption{The mAP@20 results for image-to-text ($I \to T$) and text-to-image ($T \to I$) retrieval for the UCM dataset when $B=64$.}
\small
\label{tab:retrieval-ucm}
\def\arraystretch{1.0}
\begin{tabular}{c|l|cccccc}
\hline
\multirow{2}{*}{Task} & \multirow{2}{*}{Metod} & \multicolumn{6}{c}{Amount of the caption noise} \\
 & & 5\% & 10\% & 20\% & 30\% & 40\% & 50\% \\
\hline\hline
\multirow{7}{*}{$I \to T$}
 & DUCH-NR-NW & \textbf{0.868} & \underline{0.843} & \underline{0.845} & \textbf{0.828} & 0.794 & 0.779 \\
 & DUCH-NR-EW & \underline{0.851} & \textbf{0.851} & \textbf{0.861} & 0.820 & \textbf{0.838} & \textbf{0.821} \\
 & DUCH-NR-DW & 0.843 & 0.832 & 0.844 & \underline{0.823} & \underline{0.821} & \underline{0.796} \\
\cline{2-8}
 & DUCH-PTC & 0.849 & 0.828 & 0.803 & 0.739 & 0.713 & 0.614 \\
 & DUCH & 0.840 & 0.822 & 0.798 & 0.727 & 0.691 & 0.557 \\
 & JDSH\cite{liu2020joint} & 0.806 & 0.775 & 0.714 & 0.620 & 0.567 & 0.396 \\
 & DJSRH\cite{su2019deep} & 0.707 & 0.688 & 0.633 & 0.586 & 0.534 & 0.426 \\
\hline\hline
\multirow{7}{*}{$T \to I$}
 & DUCH-NR-NW & 0.921 & \underline{0.912} & \underline{0.907} & 0.883 & 0.855 & 0.810 \\
 & DUCH-NR-EW & 0.915 & \textbf{0.917} & 0.902 & \textbf{0.896} & \underline{0.882} & \textbf{0.875} \\
 & DUCH-NR-DW & \textbf{0.929} & \underline{0.912} & \textbf{0.908} & \underline{0.891} & \textbf{0.885} & \underline{0.849} \\
\cline{2-8}
 & DUCH-PTC & 0.911 & 0.907 & 0.869 & 0.850 & 0.765 & 0.688 \\
 & DUCH & \underline{0.925} & 0.905 & 0.881 & 0.821 & 0.738 & 0.641 \\
 & JDSH\cite{liu2020joint} & 0.882 & 0.860 & 0.764 & 0.699 & 0.603 & 0.442 \\
 & DJSRH\cite{su2019deep} & 0.751 & 0.742 & 0.685 & 0.621 & 0.521 & 0.468 \\
\hline
\end{tabular}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/noise_rsicd_0.2_i2t.pdf}
        \caption[]
        {}    %{\small Gaussian blur with kernel size $3 \times 3$.}
        \label{fig:retrieval-rsicd-i2t}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{images/noise_rsicd_0.2_t2i.pdf}
        \caption[]
        {}    %{\small Random rotation in given range.}
        \label{fig:retrieval-rsicd-t2i}
    \end{subfigure}
    \caption[]{\small Image-to-text (a) and text-to-image (b) mean average precision for top-20 samples (mAP@20) versus noise probability of the data for the RSICD dataset when $B$=64} 
    \label{fig:retrieval-rsicd}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/noise_ucm_0.3_i2t.pdf}
        \caption[]
        {}    %{\small Gaussian blur with kernel size $3 \times 3$.}
        \label{fig:retrieval-ucm-i2t}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{images/noise_ucm_0.3_t2i.pdf}
        \caption[]
        {}    %{\small Random rotation in given range.}
        \label{fig:retrieval-ucm-t2i}
    \end{subfigure}
    \caption[]{\small Image-to-text (a) and text-to-image (b) mean average precision for top-20 samples (mAP@20) versus noise probability of the data for the UCM dataset when $B$=64} 
    \label{fig:retrieval-ucm}
\end{figure}
